MDP: Multidimensional Vision Model Pruning with Latency Constraint

Current structural pruning methods face two significant limitations: (i) they often limit pruning to finer-grained levels like channels, making aggressive parameter reduction challenging, and (ii) they focus heavily on parameter and FLOP reduction, with existing latency-aware methods frequently relying on simplistic, suboptimal linear models that fail to generalize well to transformers, where multiple interacting dimensions impact latency. In this paper, we address both limitations by introducing Multi-Dimensional Pruning (MDP), a novel paradigm that jointly optimizes across a variety of pruning granularities-including channels, query, key, heads, embeddings, and blocks. MDP employs an advanced latency modeling technique to accurately capture latency variations across all prunable dimensions, achieving an optimal balance between latency and accuracy. By reformulating pruning as a Mixed-Integer Nonlinear Program (MINLP), MDP efficiently identifies the optimal pruned structure across all prunable dimensions while respecting latency constraints. This versatile framework supports both CNNs and transformers. Extensive experiments demonstrate that MDP significantly outperforms previous methods, especially at high pruning ratios. On ImageNet, MDP achieves a 28% speed increase with a +1.4 Top-1 accuracy improvement over prior work like HALP for ResNet50 pruning. Against the latest transformer pruning method, Isomorphic, MDP delivers an additional 37% acceleration with a +0.7 Top-1 accuracy improvement.

==> preamble.tex <==
%
% --- inline annotations
%
\usepackage[dvipsnames, table]{xcolor}
% \usepackage[table]{xcolor}
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
\newcommand{\alex}[1]{\textbf{\color{red}[alex: #1]}}
\definecolor{lgreen}{RGB}{236, 255, 201}
\definecolor{nvgreen}{RGB}{118, 185, 0}
\definecolor{cvprblue}{rgb}{0.21,0.49,0.74}
\definecolor{lgray}{RGB}{245,245,245}

\definecolor{lightblue}{rgb}{0.678, 0.847, 0.902}
\definecolor{coral}{rgb}{1.0, 0.498, 0.314}
\definecolor{mint}{rgb}{0.686, 0.933, 0.651}
\definecolor{lavender}{rgb}{0.902, 0.902, 0.980}
\definecolor{peach}{rgb}{1.0, 0.855, 0.725}
\definecolor{teal}{rgb}{0.0, 0.502, 0.502}
\definecolor{gold}{rgb}{1.0, 0.843, 0.0}
\definecolor{skyblue}{rgb}{0.529, 0.808, 0.922}
\definecolor{salmon}{rgb}{0.980, 0.502, 0.447}
\definecolor{orchid}{rgb}{0.854, 0.439, 0.839}
\definecolor{plum}{rgb}{0.867, 0.627, 0.867}
\definecolor{chartreuse}{rgb}{0.498, 1.0, 0.0}
\definecolor{crimson}{rgb}{0.862, 0.078, 0.235}
\definecolor{khaki}{rgb}{0.941, 0.902, 0.549}

\newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}%
\usepackage{amsmath}
\usepackage{pifont}% http://ctan.org/pkg/pifont
\usepackage{float}
\usepackage{arydshln}
\usepackage{algorithm}
\usepackage{algorithmicx}
\usepackage{algpseudocode}
\usepackage{subcaption}
\usepackage{cuted}
\usepackage{bm}
\usepackage{dsfont}
\setcounter{secnumdepth}{4}
\algrenewcommand\alglinenumber[1]{\tiny #1:}
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

==> sec/1_intro_bullet.tex <==
\section{Introduction}
\textbf{Background:} DNNs have become the de-facto. We have seen both CNNs and transformers thriving. Also, these models are getting bigger in size, creating challenges for hardware.

\begin{figure*}[t!]
    \centering
    \includegraphics[width=\linewidth]{figs/MDP-framework.pdf}
    \caption{Paradigm of our proposed method. We start by computing layer importance and constructing latency cost matrices for each layer. We then group layers within the same block and solve an MINLP to optimize pruning decisions at both channel and block levels. Finally, we extract the pruned subnetwork and finetune it.}
    \label{fig:paradigm}
\end{figure*}

\textbf{Previous methods and limitation:} Structural pruning has shown to be a promising method to effectively reduce computation for either CNN or transformer. However, two major limitations:

1. Approaches usually only tackle moderate pruning ratios. Fall short with larger pruning since they can not handle block or layer (structural) removal. 

2. Current methods that directly reduce inference latency (e.g. HALP, etc.) only focus on CNNs; even though CNNs latency estimation is also frequently inaccurate. 

\textbf{Our contribution:}
% they are infeasible with pruning transformer since it lacks the ability to monitor the variations across multiple dimensions (e.g. query, value, MLP, embedding, etc.); existing latency aware transformer pruning works only use latency as a regularization and can’t be exact.
To overcome the above two issues, we identify the issue lies in the inability to simultaneously handle multiple dimensions during pruning. We also incorporate layer and block as “group” to simultaneously determine optimal sparse architectures on both channel and block levels to enable large-ratio pruning. We propose an accurate latency modeling technique to simultaneously monitor the latency variation of the model across multiple different dimensions. With the above steps, we innovatiyle reformulate pruning as a Mixed-Integer Nonlinear Program (MINLP) optimization then solve it with modern numerical optimization frameworks.

1. we introduce a method to enable simultaneous channel and block pruning, allowing collective decision-making in optimization.

2. we propose an accurate latency formulation method that could simultaneously capture the variations across multiple dimensions

3. We are the first in the field that achieves exact latency-constrained pruning for transformers

4. we organically combine all above into a MINLP

5. experiments are conducted and show great results




==> sec/2_related_bullet.tex <==
% A plethora of pruning methods has yielded profound progresses in model compression~\cite{lecun1990optimal, han2015deep, gale2019state, zhou2021effective, sun2022disparse}, providing practical speedup and memory benefits~\cite{li2017pruning, molchanov2019importance, he2020learning, lin2020hrank} through hardware-friendly sparsity~\cite{wu2020constraint, li2020eagleeye, shen2021halp, humble2022soft, shen2023hardware} that trades off accuracy and performance  via FLOPs/latency. Our work can be categorized into the field of model pruning. In this section, we will provide a recap of pruning and discuss the latest methods in the field.
\section{Related Works}
\label{sec:related}
Our work can be categorized as a pruning method. 
\textbf{Channel Pruning}
  \begin{enumerate}
      \item A brief overview of the field. Then introduce channel pruning.
  \end{enumerate}
  
\noindent\textbf{Layer and Block Pruning}
\begin{enumerate}
    \item Explain that channel pruning is only limited to channel level and a moderate pruning ratio. At large pruning ratio, we need to remove block and layer.
    \item Not a lot of works focusing on this. Cite the few works in this direction. 
    \item Mention alternative ways to achieve this. Some automl and NAS approaches. Rely on a very computationally expensive searching and enumeration process.
    \item Discuss our difference. We do not need any training from scratch and tackle from an optimization perspective. We consider layer and block as "group" in optimization.
\end{enumerate}


\noindent\textbf{Hardware-aware Pruning} Since both parameter counts or FLOPs do not directly translate into latency, latest methods go one step further and perform hardware-aware pruning which aims to directly reduce the hardware inference latency. 
\begin{enumerate}
    \item Mention and describe the HALP, SMCP, and the IV paper. Discuss how they set up the Knapsack problem to solve the pruning objective.
    \item Discuss their limitations. Latency estimation is inaccurate. Describe that only latency impact from reducing output channels is considered, but neglecting simultaneous variations in both input and output. (Concretely, when we prune output channels for a layer, the input channel count for its connected subsequent layer also changes, but this is not captured. Mention we show detailed formulation in Appendix to explain this.)
    \item Discuss our differences. We introduce layer latency matrix to simultaneously capture the impacts on latency from both input and output channel levels and globally solve the optimal channel counts for all layers with joint optimization.
\end{enumerate}

\noindent\textbf{Mixed-Integer Nonlinear Program (MINLP)~\cite{lee2011mixed, burer2012non, bussieck2003mixed}} Since the backbone of our proposed formulation is a MINLP, we will now briefly introduce the field. 
\begin{enumerate}
    \item Explain the definition of MINLP
    \item What are the common solvers for MINLP?
    \item Which solver do we use?
\end{enumerate}
  
  % Though achieving decent accuracy and speedups on various datasets, these methods~\cite{shen2021halp, shen2023hardware, humble2022soft} start to exhibit severe performance drops with large latency reduction ratio or one-shot pruning, which are limited by two main criteria. First, their optimization framework itself is inaccurate and does not include all variables affecting parameter latency. For example, inference latency of a convolution layer can be characterized by two prunable parameters: number of input channels and output channels, whereas they~\cite{shen2021halp, humble2022soft, shen2023hardware} only include the number of output channels into their mathematical modeling. Second, they are incapable of handling hierarchical changes in pruning, like the removal of an entire residual block. Notably, we find that this hierarchical unawareness is also a common issue in almost all other pruning methods~\cite{molchanov2019importance, he2019filter, lin2020hrank, wimmer2022interspace, li2023differentiable}. Our work also focuses on the hardware-aware pruning setting and presents a novel pruning framework that effectively addresses the above issues.


==> sec/3_method_bullet.tex <==
\section{Methodology}
\noindent\textbf{Notations}
\begin{enumerate}
    \item Define some terms and expressions
    \item Use a table to declare notations. More organized and clear.
    \item Explain each notation briefly.
\end{enumerate}

\subsection{Method Name}
State our problem. Go over the method. Our method consists of four steps. Given a pretrained model and a desired latency budget, we simply carry out the following four steps.

Here we will describe each of the four stages in our algorithm. 

\noindent\textbf{Step 1: Compute Configuration Importance.}
\begin{enumerate}
    \item Discuss how we measure channel importance score
    \item Discuss how we go from channel importance score to layer configuration importance
\end{enumerate}
\noindent\textbf{Step 2: Construct Latency Matrices.}
\begin{enumerate}
    \item Discuss how we construct the latency matrix for each layer from a lookup table
    \item \textit{This is one of our important features.} Discuss how this captures variations in both input and output channels, and a bit comparison with HALP.
\end{enumerate}

\noindent\textbf{Step 3: Group Block}
\begin{enumerate}
    \item Discuss how we group channels belonging to the same block together.
    \item \textit{This is one of our important features.} Discuss what this grouping will do in optimization, and what benefits come from this?
\end{enumerate}

\noindent\textbf{Step 4: Solve MINLP}
\begin{enumerate}
    \item Present the optimization problem we solve
    \item Discuss how to input it into the MINLP solver
    \item Discuss a few constraints we need to consider.
\end{enumerate}

Present the pseudo code.
% Although we prevent layers from getting completely pruned, the block decision variables with higher priority will remove the entire 

==> sec/4_exp_bullet.tex <==
\section{Experiments}

To validate our proposed method, we perform extensive experiments across a comprehensive set of scenarios. 
\begin{enumerate}
    \item  Results on the image classification task with ImageNet~\cite{deng2009imagenet} and ResNet50~\cite{he2016deep}
    \item 2D object detection task with Pascal VOC~\cite{everingham2010pascal}
    \item 3D object detection task with Nuscenes~\cite{caesar2020nuscenes} and StreamPETR~\cite{wang2023exploring}
    \item Discuss baselines we compare. Under what settings
    \item Also conducted an in-depth ablation study, highlighting the contributions of our block grouping and more accurate latency pruning individually.
\end{enumerate}

Go over the optimization and experiment settings. On what device, PyTorch, GPU...

\textbf{Results on ImageNet}
\begin{enumerate}
    \item Table~\ref{table:imageresnet50}
    \item Describe evaluation metrics
    \item Discuss the results. Particularly compared with HALP and SMCP.
    \item Particularly excels when targeting high FPS at aggressive pruning ratio, validating the effectiveness.
\end{enumerate}

\begin{table*}[ht!]
    \centering
    \vspace{-0.2cm}
    % \resizebox{.85\textwidth}{!}
    {
        % \begin{tabular}{c|cccc}
        \begin{tabular}{lcccc}
            \toprule
            \rowcolor{lgray} 
            \textsc{Method} & \textsc{Top-1 Acc}($\%$)$\uparrow$ & \textsc{Top-5 Acc}($\%$)$\uparrow$  & \textsc{FLOPs}($\times e^9$)$\downarrow$ & \textsc{FPS(im/s)}$\uparrow$ \\
            % {\footnotesize (baseline)}
            \midrule
            \multicolumn{5}{c}{\textbf{ResNet50~\cite{he2016deep}}}\\
            \textsc{Dense} & $76.2$&$92.9$ & $4.1$&$1019$\\
            \midrule
            \textsc{MetaPrune}\cite{liu2019metapruning} & $73.4$ & --& $1.0$ & $2381$ \\
            \textsc{AutoSlim}\cite{yu2019autoslim} & $74.0$ & --& $1.0$ & $2390$ \\
            \textsc{GReg-2}\cite{wang2021neural} & $73.9$ & --& $1.3$ & $1514$ \\
            \textsc{HALP-$30\%$}\cite{shen2021halp} & $74.5$ &$91.8$ & $1.2$ & $2597$ \\
            \textsc{SMCP-$30\%$}\cite{humble2022soft} & $\mathbf{74.6}$ &$92.0$ & $1.0$ & $2947$ \\
            %\textsc{HALP*-$30\%$} & $74.5$ &$92.0$& $1.1$ & $2488$ & $90+90$&\cmark\\
            \rowcolor{lgreen} \textbf{\textsc{Ours-30\%}} & $\mathbf{74.6}$ &$\mathbf{92.2}$ & $1.1$ & $\mathbf{3092}$ \\
            \midrule
            \textsc{HALP-$15\%$}\cite{shen2021halp} & $68.1$ &$88.4$& $0.6$ & $3971$ \\
            \rowcolor{lgreen} \textbf{\textsc{Ours-15\%}} & $\mathbf{70.0}$ &$\mathbf{89.3}$& $0.5$ & $\mathbf{5306}$ \\
            \midrule
            \midrule
            \multicolumn{5}{c}{\textbf{ResNet50 - EagleEye~\cite{li2020eagleeye}}}\\
            \textsc{Dense}~\cite{li2020eagleeye} & $77.2$ &$93.7$& $4.1$&$1019$\\
            \bottomrule
 \textsc{EagleEye-1G}\cite{li2020eagleeye} & $74.2$ &$91.8$ & $1.0$ & $2429$ \\
 \textsc{HALP-30\%}\cite{shen2021halp} & $74.5$ &$91.9$ & $1.2$ & $2597$ \\
  \textsc{SMCP-30\%}\cite{humble2022soft} & $75.1$ &$92.3$ & $1.1$ & $2589$ \\
    \rowcolor{lgreen}
  \textbf{\textsc{Ours-35\%}} & $\mathbf{75.2}$ &$\mathbf{92.5}$& $1.3$ & $\mathbf{2774}$ \\
  \rowcolor{lgreen}
  \textbf{\textsc{Ours-30\%}} & $75.0$ &$92.2$& $1.2$ & $3052$ \\
  \midrule
  % \textsc{SMCP-25\%}\cite{humble2022soft} & $74.4$ &$92.0$ & $0.9$ & $3102$ \\
  \textsc{HALP-20\%}\cite{shen2021halp} & $71.2$ &$90.1$& $0.7$ & $3691$ \\
  \textsc{SMCP-20\%}\cite{humble2022soft} & $72.7$ &--& --& $3784$ \\
  \rowcolor{lgreen}
  \textbf{\textsc{Ours-20\%}} & $\mathbf{72.8}$ &$\mathbf{90.9}$& $0.7$ & $\mathbf{4210}$ \\
  \midrule
\textsc{HALP-15\%}\cite{shen2021halp} & $68.6$ &$88.5$& $0.6$ & $4101$ \\
\rowcolor{lgreen}
\textbf{\textsc{Ours-15\%}} & $\mathbf{70.0}$ &$\mathbf{89.2}$& $0.5$ & $\mathbf{5262}$ \\
\bottomrule
        \end{tabular}
    }
    \caption{\textbf{ImageNet results with ResNet-50}. FPS is measured on NVIDIA TITAN V. Results with similar FPS are grouped. Ours achieve much better accuracy-FPS tradeoffs than the baselines, specifically when pruning ratio is large. Averaged results over two runs.}
    \label{table:imageresnet50}
\end{table*}

\begin{figure}[ht!]
\begin{center}
   \includegraphics[width=.5\linewidth]{figs/pascalvoc.pdf}
\end{center}
\vspace{-5pt}
\caption{\textbf{PascalVOC results with SSD512}. Results of FPS versus mAP are plotted (left, top-right is better). FPS is measured on NVIDIA TITAN V. Ours achieve much better accuracy-FPS tradeoffs than the baselines.}
\label{fig:pascal}
\end{figure}
\textbf{Results on PascalVOC} 
\begin{enumerate}
    \item Figure~\ref{fig:pascal}
    \item Describe evaluation metrics
    \item Describe the Pareto Frontier is much better. Discuss the results and compare with SMCP.
\end{enumerate}

\begin{table*}[ht!]
\centering
\begin{tabular}{c|c|c|ccccc|c}
\toprule
\rowcolor{lgray}
\textsc{Method} & \textsc{mAP$\uparrow$} & \textsc{NDS$\uparrow$} & \textsc{mATE$\downarrow$} & \textsc{mASE$\downarrow$} & \textsc{mAOE$\downarrow$} & \textsc{mAVE$\downarrow$} & \textsc{mAAE$\downarrow$} & \textsc{FPS$\uparrow$} \\
\midrule
\textsc{BEVPoolv2}\cite{huang2022bevpoolv2} & $0.406$ & $0.526$ & $0.572$ & $0.275$ & $0.463$ & $0.275$ & $0.188$ & $16.6$ \\
\textsc{BEVDet4D}\cite{huang2022bevdet4d}& $0.322$ & $0.457$ & $0.703$ & $0.278$ & $0.495$ & $0.354$ & $0.206$ & $16.7$ \\
\textsc{PETRv2}\cite{liu2023petrv2} & $0.349$ & $0.456$ & $0.700$ & $0.275$ & $0.580$ & $0.437$ & $0.187$ & $18.9$ \\
\textsc{Sparse4Dv2}\cite{lin2023sparse4d} & $0.439$ & $0.539$ & $0.598$ & $0.270$ & $0.475$ & $0.282$ & $0.179$ & $20.3$ \\
\textsc{StreamPETR}\cite{wang2023exploring} & $0.449$ & $0.546$ & $0.613$ & $0.267$ & $0.413$ & $0.265$ & $0.196$ & $31.7$ \\
\rowcolor{lgreen}
\textbf{\textsc{Ours-55\%}} & $\mathbf{0.451}$ & $\mathbf{0.551}$ & 0.596& 0.272& 0.413& $0.259$& $0.207$& $\mathbf{37.3}$ \\
\midrule
\textsc{HALP-50\%}~\cite{shen2021halp} & $0.439$ & $0.543$ & 0.605 & 0.270 & 0.419 & 0.265 & 0.211 & $38.6$ \\
\rowcolor{lgreen}
\textbf{\textsc{Ours-50\%}} & $\mathbf{0.441}$ & $\mathbf{0.544}$ & 0.606 & 0.269 & 0.421 & 0.268 & 0.205& $\mathbf{39.0}$ \\
\midrule
\textsc{HALP-40\%}~\cite{shen2021halp} & $\mathbf{0.427}$ & $\mathbf{0.533}$ & 0.620 & 0.269 & 0.438 & 0.271 &0.209 &$39.5$ \\
\rowcolor{lgreen}
\textbf{\textsc{Ours-40\%}} & $\mathbf{0.427}$ & $0.532$ & 0.608 &  0.272 & 0.457 &0.269 &0.207 & $\mathbf{40.7}$ \\
\midrule
\textsc{HALP-30\%}~\cite{shen2021halp} & $0.373$ & $0.489$ & 0.674 & 0.277 & 0.534 & 0.293 & 0.197 & $42.5$ \\
\rowcolor{lgreen}
\textbf{\textsc{Ours-30\%}} & $\mathbf{0.394}$ & $\mathbf{0.512}$ & 0.642 & 0.275 & 0.449 & 0.278 & 0.204 & $\mathbf{43.3}$ \\
\bottomrule
\end{tabular}
\caption{\textbf{Nuscenes results with StreamPETR}. FPS is measured on NVIDIA GeForce RTX 3090. Results with similar FPS are grouped. Ours achieve much better accuracy-FPS tradeoffs than HALP and even surpass performance of dense StreamPETR with much higher FPS.}
\label{table:nuscenes}
\end{table*}
\textbf{Results on Nuscenes}
\begin{enumerate}
    \item Motivate again why we show this result. This is on the very latest modern 3D detection model with transformers. Our algorithm could enhance the accuracy-latency even for this hybrid structure. Report FPS of CNNs v.s. Transformers from SteamPETR.
    \item Table ~\ref{table:nuscenes}
    \item Describe evaluation metrics
    \item Discuss the results. Compared with HALP, the advantage is more obvious at large pruning, again validating our effectiveness.
    \item Even improve baseline StreamPETR result with the $-55\%$ settings.
\end{enumerate}

\subsection{Ablation Study}
Explain how we conduct ablation. Compared with pruning methods like HALP, our features are:
\begin{enumerate}
    \item Block Grouping
    \item Layer Latency Matrices
\end{enumerate}
We ablate each of them to study individual effects.


\noindent\textbf{Block Grouping}
\begin{enumerate}
    \item Figure \ref{fig:ablation}
    \item Discuss how this setting is run. Relate to the Methodology section.
    \item Discuss the results. Block grouping individually brings benefits.
    \item \alex{Maybe we also add another plot showing the pruned structure distribution here. Or this can be included in the Appendix?}
\end{enumerate}

\noindent\textbf{Layer Latency Matrices}
\begin{enumerate}
    \item Figure \ref{fig:ablation}
    \item Discuss how this setting is run. Relate to the Methodology section.
    \item Discuss the results. Using layer latency matrices individually brings benefits.
\end{enumerate}

\noindent\textbf{One-shot versus Iterative Pruning} 
\begin{enumerate}
    \item Discuss if we use iterative pruning for our setting instead what will be the difference.
    \item \alex{Figure \ref{fig:ablation} missing one line}
    \item Table \ref{table:ablation} goes into a bit more detail and study how different steps affect the performance. HALP collapses with one shot.
\end{enumerate}


\begin{table}[t!]
\centering
\begin{tabular}{c|clcc}
\toprule
\rowcolor{lgray}
\textsc{Method} & \textsc{Steps} &\textsc{Ratio}& \textsc{Top-1$\uparrow$}& \textsc{FPS$\uparrow$} \\
\midrule
\textsc{HALP}\cite{shen2021halp} & $30$  &70& $74.3$ & $2505$ \\
\textsc{HALP}\cite{shen2021halp} & $10$  &70& $73.9$ & $2622$ \\
\textsc{HALP}\cite{shen2021halp} & $1$  &70& $65.1$ & $4444$ \\
\hdashline
\textbf{\textsc{Ours}} & $30$  &70& $74.5$ & $2660$ \\
\textbf{\textsc{Ours}} & $10$  &70& $74.8$ & $2860$ \\
\rowcolor{lgreen}
\textbf{\textsc{Ours}} & $1$  &70& $75.2$ & $2774$ \\
\bottomrule
\end{tabular}
\caption{\textbf{Ablation study results on ImageNet with ResNet50}. Results of HALP~\cite{shen2021halp} and ours with different pruning steps are shown with a pruning ratio of $70\%$. One-shot pruning correspond to Steps of 1. HALP is completely not functioning with one-shot or smaller pruning steps.}
\label{table:ablation}
\end{table}

\begin{figure}[t!]
\begin{center}
   \includegraphics[width=.5\linewidth]{figs/Ablation3.pdf}
\end{center}
\vspace{-5pt}
\caption{\textbf{Abaltion study results on ImageNet with ResNet50}. We ablate on our method and show the results of each component of our formulation operating independently. Top-right is better.}
\label{fig:ablation}
\end{figure}

==> sec/6_sup.tex <==
\clearpage
% \setcounter{section}{0}
\renewcommand*{\thesection}{\Alph{section}}
\setcounter{section}{0}
\textbf{\large Appendix}
\section{Detailed Analysis on Prior Latency Estimation}
In the main paper, we note that previous approaches~\cite{shen2021halp, shen2023hardware, humble2022soft} use an imprecise estimation of latency, resulting in suboptimal trade-offs between accuracy and latency. These methods consider changes in output channels but ignore concurrent variations in input channels that occur due to pruning the previous layer. This problem becomes more significant when targeting substantial reductions in latency. In this section, we will examine their limitations through detailed formulations.

To model the latency variations, previous methods compute a latency cost for the $j$-th channel at the $l$-th layer $\Theta_l^j$ as:
\begin{align}
\label{eqn: latency}
    R_l^j = T_l(p_{l-1}, j) - T_l(p_{l-1}, j-1)
\end{align}
Here, $T(.)$ is the pre-built lookup table, and $T_l(i, j)$ returns the latency of layer $l$ with $i$ input channels and $j$ output channels. Since previous methods leverage an iterative pruning technique to gradually reach the desired latency target, $p_{l-1}$ is the \textbf{total} number of input channels kept from the last pruning step. It is used as a constant input channel count in the current pruning step to query the latency from the lookup table $T_l$. However, we can not ascertain that the input channel count will remain the same throughout the current pruning step, which can only happen if previous layer is not pruned at all. The actual value of input channel count $\hat{p}_{l-1}$ will be smaller than this constant estimate $p_{l-1}$ if pruning takes place in the previous layer. Therefore, we have the following inequalities:
\begin{align}
    \hat{p}_{l-1} &\leq p_{l-1}\\
    T_l(\hat{p}_{l-1}, j) &\leq T_l(p_{l-1}, j)\\
    T_l(\hat{p}_{l-1}, j-1) &\leq T_l(p_{l-1}, j-1)
\end{align}

We can write the error of the latency estimation for each channel from the true value as:
\begin{align}
    \epsilon_l^j &= |\hat{R}_l^j - R_l^j| \\
    &= |T_l(\hat{p}_{l-1}, j) - T_l(\hat{p}_{l-1}, j-1) - T_l(p_{l-1}, j) + T_l(p_{l-1}, j-1)|\\
    &= |(T_l(p_{l-1}, j-1) - T_l(\hat{p}_{l-1}, j-1)) + (T_l(\hat{p}_{l-1}, j) - T_l(p_{l-1}, j))| \\
    &\leq |T_l(p_{l-1}, j-1) - T_l(\hat{p}_{l-1}, j-1)| + |T_l(p_{l-1}, j) + T_l(\hat{p}_{l-1}, j)|
\end{align}
When targeting large pruning ratio, the difference between $p_{l-1}$ and $\hat{p}_{l-1}$ will be enlarged since we expect to aggressively prune each layer and the input channel count will change substantially overtime. We could see from the formula that this latency modeling will be much more prone to make mistakes in measuring the channel latency cost under such scenarios.

In terms of our proposed latency estimation technique, instead of capturing latency cost for each channel, we directly model the latency for all configurations with differing input and output channel counts to enumerate the entire latency landscape at layer $l$. Recall our latency cost matrix $\mathbf{C}_l$ looks like:
\begin{align}
{
  \mathbf{C}_l =
  \left[ {\begin{array}{cccc}
    T_l(1,1) & T_l(1,2)& \cdots & T_l(1,m_l)\\
    T_l(2, 1) & T_l(2,2) & \cdots & T_l(2, m_l)\\
    \vdots & \vdots & \ddots & \vdots\\
    T_l(m_{l-1}, 1) & T_l(m_{l-1}, 2) & \cdots & T_l(m_{l-1}, m_l)\\
  \end{array} } \right]
}
\end{align}

Previous approaches could be viewed as \textbf{only leveraging the $p_{l-1}$th row of $\mathbf{C}_l$}:
\begin{align}
{
  \left[ {\begin{array}{cccc}
    T_l(p_{l-1},1) & T_l(p_{l-1},2)& \cdots & T_l(p_{l-1},m_l)\\
  \end{array} } \right]
}
\end{align}.

\section{Solving MINLPs}
In order to solve our MINLP program, we leverage the method called OA~\cite{duran1986outer,fletcher1994solving} which decomposes the problem into solving an alternating finite sequence of NLP subproblems and relaxed versions of MILP master program. We also leverage a method called Feasibility Pump~\cite{bonami2009feasibility} to   to expedite the process of finding feasible solutions within constraints. 

The entire program could be efficiently solved on common CPUs for modern network sizes. For instance, when applied to a model like ResNet50~\cite{he2016deep}, the entire optimization problem can be solved in approximately 5 seconds on an Intel Xeon E5-2698 CPU.


\begin{figure}[t!]
  \begin{minipage}[h]{.54\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figs/pruned_structure.png}
    \vspace{-20pt}
    \captionof{figure}{Pruned architecture.}
    \label{fig:pruned_arch}
  \end{minipage}
  \hfill
  \begin{minipage}[h]{.44\linewidth}
    \centering
    \resizebox{\linewidth}{!}
    {
        \begin{tabular}{c|cc}
            \toprule
            \rowcolor{lgray}
            \textsc{Method} & \textsc{Top-1} & \textsc{FPS}\\
            \textsc{Autoslim}[\textcolor{eccvblue}{67}] & $74.0$  & $33.3$\\
            \textsc{EagleEye}[\textcolor{eccvblue}{36}] & $74.2$  & $31.3$\\
            \textsc{MetaPrune}[\textcolor{eccvblue}{43}] & $73.4$  & $33.3$\\
            \textsc{HALP}-$70\%$[\textcolor{eccvblue}{52}] & $74.5$  & $45.9$\\
            \rowcolor{lgreen}
            \textbf{Ours} & $\mathbf{75.2}$ & $\mathbf{118.2}$ \\
            \bottomrule
        \end{tabular}
    }
      \captionof{table}{Results on Intel CPU Xeon E5.}
      \label{table:cpu}
    \end{minipage}
    \vspace{-12pt}
\end{figure}

\section{Pruned Architecture} To gain deeper understanding of our pruning framework, we demonstrate the pruned structure in Fig.~\ref{fig:pruned_arch}. Our optimization approach maximizes global importance of a neural network under user-defined latency constraint (Eqn.\ref{eqn:program}), eliminating the need to pre-define pruning ratios. This automatically finds the optimal solution, pruning blocks only if their impact on overall importance is minimal compared to other options. The resulting pruned structure (Fig. \ref{fig:pruned_arch}) reveals that pruning is concentrated in shallower layers, contrary to the general expectation of layer collapse in deeper layers due to smaller gradients. 

\section{Performance on CPU Platform}
% To demonstrate the adaptability and effectiveness of our approach across platforms, we evaluated our method targeting to optimize latency on \textbf{CPU} platform of Intel Xeon E5. Results \textbf{(Table \ref{table:cpu})} demonstrate significant performance improvements over prior work. Concretely, compared with HALP~\cite{shen2021halp}, we surpass its Top-1($75.2$ v.s. $74.5$) while more than doubling its FPS($118.2$ v.s. $45.9$). This improvement is even more pronounced than our GPU results shown in the main paper. We attribute this to our framework's ability of pruning blocks, leading to a shallower structure is more friendly to CPU inference. This further validates our potential for widespread applicability. Algorithm wise, to enable different latency optimization target(e.g. CPU v.s. GPU), our framework simply requires producing a latency lookup table $\mathcal{T}_l$ (\textit{Section 3.1 Latency Modeling}) on the target platform, and feed it into the MINLP program.
To demonstrate the adaptability and effectiveness of our approach across platforms, we instantiated and evaluated our method with the goal of optimizing latency on the Intel Xeon E5 CPU. The results, shown in Table \ref{table:cpu}, demonstrate significant performance improvements over previous work. Specifically, compared to HALP~\cite{shen2021halp}, we achieve higher Top-1 accuracy (75.2 vs. 74.5) while more than doubling the FPS (118.2 vs. 45.9). This improvement is even more pronounced than our GPU results presented in the main paper. We attribute this to our framework's ability to prune blocks, resulting in a shallower structure that is more conducive to CPU inference. This further underscores our method's potential for widespread applicability. Algorithmically, to enable different latency optimization targets (e.g., CPU vs. GPU), our framework only requires generating a latency lookup table $\mathcal{T}_l$ (\textit{Section 3.1 Latency Modeling}) on the target platform and feeding it into the MINLP program.

\section{Integration with Soft Masking}
Recent advances in pruning~\cite{humble2022soft, zhou2021learning, he2018soft, kusupati2020soft, kim2021dynamic} have increasingly adopted soft masking techniques to retain the learning capacity of pruned models by not directly removing the pruned weights. Notably, SMCP~\cite{humble2022soft} integrates this method into the HALP hardware-aware pruning framework, resulting in an enhanced accuracy-latency tradeoff for pruned models. Here, we explore the potential of soft masking to enhance our model's performance. 

We conduct this study on ImageNet with ResNet50 and depict the Pareto frontier of FPS versus Top-1 in Figure~\ref{fig:softmaskg}. For clarity, we also include the performance of SMCP~\cite{humble2022soft} and ours. The results reveal that soft masking offers limited advantages at lower FPS levels with modest pruning ratios and latency reduction. Nonetheless, targeting higher FPS levels leads to notable improvements in Top-1 accuracy. This outcome may be attributed to the Taylor channel importance score we employed~\cite{molchanov2019importance}, which gauges parameter significance based on its impact on loss. Though it maintains precision with minor parameter deletions, its reliability may diminish when a larger number of parameters are pruned concurrently. The iterative reassessment inherent to the soft masking technique may counteract this shortcoming.


\begin{figure}[h!]
\begin{subfigure}[b]{.55\textwidth}
\begin{center}
   \includegraphics[width=\linewidth]{figs/ComparisonWithSmall.pdf}
\end{center}
\caption{\textbf{Comparison with smaller networks on ImageNet with pruning ResNet50}. Our approach of pruning large models across various ratios achieves a superior accuracy-speed trade-off compared to existing smaller networks. Top-right is better.}
\label{fig:smallarch}
\end{subfigure}
\hfill
\begin{subfigure}[b]{.45\textwidth}
\begin{center}
   \includegraphics[width=.9\linewidth]{figs/Softmasking.pdf}
\end{center}
\caption{\textbf{Results of ours with soft masking on ImageNet with ResNet50}. Improvement is observed in Top1 at a high FPS level. Top-right is better.}
\label{fig:softmaskg}
\end{subfigure}
\end{figure}

% \begin{figure}[t!]
% \begin{center}
%    \includegraphics[width=.7\linewidth]{figs/Softmasking.pdf}
% \end{center}
% \vspace{-5pt}
% \caption{\textbf{Results of ours with soft masking on ImageNet with ResNet50}. We investigate the effectiveness of soft masking techniques in our method and observe improvement in Top1 at a high FPS level. Top-right is better.}
% \label{fig:softmaskg}
% \end{figure}

\section{Comparison with Smaller Networks} In our paper, we adopt a \textit{\textbf{"training large - pruning to small"}} paradigm. Our approach is particularly effective at large pruning ratios. Therefore, instead of starting with and pruning smaller architectures like MobileNet, EfficientNet, and ResNet18, we \textbf{\textit{aggressively}} prune a larger portion from ResNet50 to attain an efficient model. This strategy outperforms other smaller networks in both Top-1 accuracy and FPS, as illustrated in Figure~\ref{fig:smallarch}. Larger networks provide a richer manifold space for learning more complex features during training compared to smaller ones, giving the pruned models greater potential. Our framework excels at identifying an optimal pruned subnetwork structure, surpassing the performance of training smaller networks from scratch.

\section{Training Detail} The hyperparameters and settings used for experiments are detailed in Table \ref{tab:detail}.
\begin{table}[H]
    \centering
    \resizebox{.99\linewidth}{!}{
    \begin{tabular}{c|ccc}
        \toprule
        \rowcolor{lgray}
        Dataset & Epochs & Optimizer, Momentum, WeightDecay & Learning Rate\\
        ImageNet & $90$  & SGD, $0.875$, $3e-5$ &Init=$1.024$, LinearDecay\\
        PascalVOC & $800$ & SGD, $0.9$, $2e-3$ &Init=$8e-3$, StepDecay \\
        NuScenes & $60$  & AdamW,$n/a$, $0.01$ & Init=$6e-4$, CosineAnneal \\
        \bottomrule
    \end{tabular}
    }
    \caption{Training Detail.}
    \label{tab:detail}
\end{table}
